Semi-verified PAC Learning from the Crowd

We study the problem of crowdsourced PAC learning of threshold functions. This is a challenging problem and only recently have query-efficient algorithms been established under the assumption that a noticeable fraction of the workers are perfect. In this work, we investigate a more challenging case where the majority may behave adversarially and the rest behave as the Massart noise - a significant generalization of the perfectness assumption. We show that under the {semi-verified model} of Charikar et al. (2017), where we have (limited) access to a trusted oracle who always returns correct annotations, it is possible to PAC learn the underlying hypothesis class with a manageable amount of label queries. Moreover, we show that the labeling cost can be drastically mitigated via the more easily obtained comparison queries. Orthogonal to recent developments in semi-verified or list-decodable learning that crucially rely on data distributional assumptions, our PAC guarantee holds by exploring the wisdom of the crowd.

==> reliable.tex <==
\section{Learning without Perfect Workers}

In this section, we elaborate on a more challenging scenario of learning from the crowd. We now have no perfect workers in the pool, but an $\alpha$-fraction of which are ``reliable''. That is, for any given instance $x$, a reliable worker $t$ can provide us the correct label $h_t(x) = h^*(x)$ with probabiltiy $1-\eta_t(x) \geq 1-\eta$, i.e. $\Pr[h_t(x)=h^*(x) \mid x] \geq 1-\eta, \forall x\in X$. We make no assumption on the remaining $(1-\alpha)$-fraction. In this case, when querying labels for any instance $x$, our purpose is to sample a large enough set of $k$ workers such that a small number of reliable workers may provide their response for $x$. As a result, the population majority size is at most
\begin{equation*}
	\smaj_{\PL}(x) \leq 1-\alpha+\eta\alpha = 1 - (1-\eta)\alpha.
\end{equation*}
Observe that if $k=\frac{32\log\frac{\abs{S}}{\delta}}{(1-\eta)^2\alpha^2}$, we have
\begin{align*}
	\Pr\[\abs{\smaj_{\WL}(x)-\smaj_{\PL}(x)} \geq\frac{(1-\eta)\alpha}{8} \] \leq e^{-2k\cdot\(\frac{(1-\eta)\alpha}{8}\)^2} \leq \frac{\delta}{\abs{S}},
\end{align*}

By setting the condition of pruning to $\smaj_{\WL}(x) \leq 1-\frac{(1-\eta)\alpha}{4}$, we are guaranteed to remove  at least a $\frac{(1-\eta)\alpha}{8}$ fraction of the workers in each pruning step. 
Unfortunately, since we have assumed that the reliable worker can also make mistake, not all the reliable workers can survive a pruning. We may prune up to $\eta$-fraction of the reliable workers from the pool as well. 
Denote by $\alpha_i$ the fraction of reliable workers and $N_i$ the number of workers in the pool after $i$ prunings. Clearly, we have $\alpha_0=\alpha$. Note that 
\begin{equation*}
\alpha_{i} N_{i} = \alpha_{i-1}N_{i-1} \cdot (1-\eta) = \dots = \alpha_{0}N_{0}\cdot (1-\eta)^{i}.
\end{equation*}
Then, we have 
\begin{align}
	\alpha_K &\geq \frac{\alpha_0 N_0\cdot\(1-\eta\)^{K}}{N_0 - \frac{(1-\eta)\alpha_0}{8}\cdot N_0 - \frac{(1-\eta)\alpha_1}{8}\cdot N_1 - \dots - \frac{(1-\eta)\alpha_{K-1}}{8}\cdot N_{K-1}} \notag\\
%	&= \frac{\alpha_0 N_0\cdot\(1-\eta\)^{K}}{N_0 - \frac{(1-\eta)}{8}\cdot \(\alpha_0N_0 + \alpha_1N_1 + \dots + \alpha_{K}N_{K}	\)} \notag\\
	&= \frac{\alpha_0 N_0\cdot\(1-\eta\)^{K}}{N_0 - \frac{(1-\eta)\alpha_0N_0}{8}\cdot \(1 + (1-\eta) + \dots + (1-\eta)^K	\)} \notag\\
	&= \frac{\alpha_0 N_0\cdot\(1-\eta\)^{K}}{N_0 - \frac{(1-\eta)\alpha_0N_0}{8}\cdot \frac{1-(1-\eta)^{K+1}}{\eta} } \notag\\
%	&= \frac{8\eta \cdot \alpha_0 \cdot\(1-\eta\)^{K}}{8\eta - (1-\eta)\alpha_0\cdot (1-(1-\eta)^{K+1}) } \\
	&= \frac{8\eta \cdot \alpha_0 \cdot\(1-\eta\)^{K}}{8\eta - \alpha_0(1-\eta) + \alpha_0(1-\eta)^{K+2} } \label{eq:alpha_K}
\end{align}

In the following, we will first consider that $\alpha_0,\eta$ are of constant scale, and see whether the pruning scheme works when no perfect is present. Followed by that, we would investigate the more challenging case when $\alpha_0,\eta$ are parameters.


{\bf Case 1: $\alpha_0,\eta$ are constants}

We first assume that all the factors $\alpha_0,\eta$ are constant. We give an example and show that our algorithm can be generalized to work on a pool of crowd workers where no perfect is presented. Without loss of generality, we set $\alpha_0=10^{-1}$ and $\eta=10^{-3}$. The purpose is to increase $\alpha_K$ until it surpasses some given constant, say $0.7$,
\begin{equation*}
	\alpha_K = \frac{8\cdot 10^{-3} \cdot 10^{-1} \cdot\(1-10^{-3}\)^{K}}{8\cdot 10^{-3} - 10^{-1}\cdot(1-10^{-3}) +  10^{-1}\cdot(1-10^{-3})^{K+2} }  \geq 0.7. 
%	&= \frac{8\cdot 10^{-3} \cdot 10^{-1} \cdot\(1-10^{-3}\)^{K}}{8\cdot 10^{-3} - 10^{-1} + 10^{-4} +  10^{-1}\cdot (1-10^{-3})^{2}\cdot(1-10^{-3})^{K} }  \\
\end{equation*}
Thus, it suffices to pick a $K$ satisfying
\begin{align}
	8\times 10^{-4} \times\(1-10^{-3}\)^{K} &\geq 0.7\times\(8.1\times 10^{-3} - 10^{-1} +  10^{-1}\times(0.999)^{2}\times(1-10^{-3})^{K}\) \\
	0.7\times 10^{-1} - 5.61\times 10^{-3} &\geq (0.07\times 0.999^2 - 8\times 10^{-4}) (1-10^{-3})^K \\
	(1-10^{-3})^K &\leq \frac{0.7\times 10^{-1} - 5.61\times 10^{-3}}{0.07\times 0.999^2 - 8\times 10^{-4}} \\
	K &\geq \log_{\frac{1000}{999}} \(\frac{0.07\times 0.999^2 - 8\times 10^{-4}}{0.7\times 10^{-1} - 5.61\times 10^{-3}}\) .
\end{align}
Notice that 
\begin{equation}
	 \frac{0.07\times 0.999^2 - 8\times 10^{-4}}{0.7\times 10^{-1} - 5.61\times 10^{-3}}  < 1.073 ,
\end{equation}
it suffices to pick $K=\log_{\frac{1000}{999}}1.073  \approx 70.4$. In other words, with at most $K=71$ pruning steps, the fraction of reliable workers $\alpha$ would surpass $0.7$, where the non-semi-verified algorithm can be invoked.


{\bf Case 2: $\alpha_0,\eta$ are parameters}

When $\alpha_0,\eta$ are not constant, there must be some conditions to be satisfied because, if $\eta$ is too large, we may remove too many reliable workers while keep most of the low-quality ones in the crowd. Without loss of generality, consider a worst case in the first pruning: the crowd workers only decrease by a $\frac{(1-\eta)\alpha}{8}$-fraction, while an $\eta$-fraction of the reliable workers are pruned. Then, if $\eta=\frac{(1-\eta)\alpha}{8}$, we would have
\begin{equation}
	\alpha_1 = \frac{\alpha_0 (1-\eta)}{1- \frac{(1-\eta)\alpha}{8}} = \frac{\alpha_0(1-\eta)}{1-\eta} = \alpha_0
\end{equation}
meaning that the fraction of the reliable workers does not improve at all. Therefore, we remark that $\eta$ must be strictly smaller than $\frac{(1-\eta)\alpha}{8}$ in every round of pruning
\begin{equation}
 \eta < \frac{(1-\eta)\alpha_i}{8}\ \forall i\geq0,
\end{equation}
since $\alpha_i\geq\alpha_0$ for any $i\geq0$, $\eta < \frac{\alpha_0}{16}$ since $1-\eta \in (\frac12,1]$.


From Eq.~\ref{eq:alpha_K}, to pick a sufficient number of verified labels $K$ that increases $\alpha_K$ to any given constant $C\in[0.7,1]$, we have
\begin{equation*}
	K \geq \log_{(1-\eta)} \frac{C\alpha_0(1-\eta) - 8C\eta}{C\alpha_0(1-\eta)^2 - 8\eta\alpha_0} 
%	=  \log_{(1-\eta)} \frac{C\alpha_0(1-\eta)^2 - 8C\eta(1-\eta)}{C\alpha_0(1-\eta)^2 - 8\eta\alpha_0} 
	= T(\alpha_0,\eta)
\end{equation*}
where $T(\alpha_0,\eta)$ is a function of variables $\alpha_0,\eta$.
%therefore, it suffices if $K$ is larger than the supreme of the right hand side of this inequality. Thus, we 
%\begin{equation*}
%	\log_{(1-\eta)} \frac{C\alpha_0(1-\eta) - 8C\eta}{C\alpha_0(1-\eta)^2 - 8\eta\alpha_0}  
%\end{equation*}
%we see that as long as $8C\eta(1-\eta) \geq 8\eta\alpha_0$, i.e. $C(1-\eta)\geq\alpha_0$ which holds naturally, $K$ is solvable. In addition, it requires $\alpha_0(1-\eta) - 8\eta>0$ for the domain of the logarithmic function, which means $\eta < \frac{\alpha_0}{\alpha_0+8}$.

Due to $C\in[0.7,1]$, $1-\eta \in (\frac12,1]$, $\alpha_0<1$, we have 
\begin{equation}
	T(\alpha_0,\eta) = O\( \log_{\frac{1}{1-\eta}}\frac{\alpha_0 - \eta\alpha_0}{\alpha_0 - \eta} \)
%	= O\( \log_{\frac{1}{1-\eta}}\frac{\alpha_0 (1- \eta)}{\alpha_0 - \eta} \) 
	= O\( \log_{\frac{1}{1-\eta}}\frac{\alpha_0}{\alpha_0 - \eta} \) 
	= O\( \log_{\frac{1}{1-\eta}}\frac{1}{\alpha_0 - \eta} \) .
%	= O\( \frac{\log (1+\frac{\eta}{\alpha_0 - \eta})}{\log (1+\eta)} \) .
\end{equation}
Notice that when $\eta \rightarrow 0$, the above term becomes
\begin{equation}
	T(\alpha_0,\eta) = \lim_{\eta\rightarrow0} O\( \frac{\log(\alpha_0 - \eta) }{\log(1-\eta)} \) = \lim_{\eta\rightarrow0} O\( \frac{1-\eta }{\alpha_0 - \eta } \) = O\(\frac{1}{\alpha_0} \),
\end{equation}
which matches with the amount as derived in Lemma~\ref{lem:restart_restate} (when $\alpha$-fraction are perfect).

%If further consider a condition that $\eta \leq \frac{\alpha_0}{c}$ for some constant $c>1$, then
%\begin{equation}
%	T(\eta) = O\(\frac{1}{\log(1+\eta)}\) .
%\end{equation}

%Analysis for pruning the adversarial workers v.s. reliable workers: one condition needs to be satisfied is that 








%Consider there are $N$ workers in the pool at the beginning of the algorithm. After $T=\frac{8}{(1-\eta)\alpha}$ prunings, the number of reliable workers remaining in the crowd is at least
%\begin{equation*}
%	 \alpha N\cdot \(1-(1-\eta)^{\frac{8}{(1-\eta)\alpha}}\) \geq   \alpha N\cdot \(1-e^{-\frac{\eta}{1-\eta}\cdot\frac{8}{\alpha}}\) \geq \alpha N\cdot\(1-e^{-\frac{8}{1-\eta}}\) \geq \alpha  N\cdot \(1-e^{-8}\)
%\end{equation*}
%where the second transition is due to the assumption that $\eta = \alpha$ and $1-\eta<1$.


==> setup.tex <==
%\section{Preliminaries}\label{sec:setup}




%\Jie{You are stating the setup, no one wants to see any of your results.}

%{Let $\X$ be the instance space and $\Y:=\{-1,+1\}$ be the label space. Let $\F$ be the class of real-valued functions $f\in\F:\X\rightarrow\R$. We refer to $\H$ as the associated {\em concept class}, specifically, a class of {\em threshold functions} $\H=\{\sign{f}:f\in\F\}$. For example, when $\F$ is the class of $\R^d\rightarrow\R$ affine functions, then the associated class $\H$ is the class of $d$-dimensional halfspaces.} Let $\D$ be a joint distribution over $\X\times\Y$ and denote by $\DX$ the marginal distribution over $\X$. We consider the {\em realizable PAC learning} setting where there is a target function $h^*$ in the hypothesis class $\H$ with zero error rate, that is, $\err_{\D}(h^*)=0$, where $\err_{\D}(h) =\Pr_{(x, y)\sim\D}(h(x)\neq y)$. In other words, the true label $y$ of a given instance $x$ is given by $y = h^*(x)$.
%Let $\X$ be the instance space, and $\Y=\{-1,+1\}$ be the set of possible labels. A {hypothesis} $h\in\H: \X\rightarrow\Y$ is a Boolean-valued function that maps an instance $x\in\X$ to its label $y$. Let $\D$ be a joint distribution over $\X\times\Y$, and denote by $\DX$ the marginal distribution on $\X$. We consider the {\em realizable PAC learning} setting where there is a target function $h^*$ in the hypothesis class $\H$ with zero error rate, that is, $\err_{\D}(h^*)=0$, where $\err_{\D}(h) =\Pr_{(x, y)\sim\D}(h(x)\neq y)$. In other words, the true label $y$ of a given instance $x$ is given by $y = h^*(x)$.

%{Following the work of \citet{shen2020learn}, we consider the learner has access to not only labels, but also pairwise comparisons. That is, for each pair of instances $(x,x')\in\X\times\X$, there is an underlying zero-error comparison function $Z^*(x,x')$ which measures the relative distance of two points to the decision boundary, i.e. $\sign{f(x)-f(x')}$.}

%We consider that the learner can query not only labels, but also pairwise comparisons. We assume that for each pair of instance $(x,x')\in\X\times\X$, there is an underlying zero-error comparison function $Z^*(x,x')$, which outputs $1$ if $x$ is more likely a positive instance than $x'$ is, and $-1$ otherwise. For example, consider the hypothesis class of halfspaces, i.e. $\H = \{h_w: x \mapsto \sign{w \cdot x}\}$ where $h_{w^*}$ has zero error rate, then the comparison function can be $Z^*(x,x') = \sign{w^* \cdot (x - x')}$.

%In this paper, we study the problem of crowdsourced PAC learning of Boolean functions through enriched queries, i.e. labels and comparison tags, when the majority of the crowd are  incorrect. We consider the {\em semi-verified} learning model of \cite{charika2017learning} where there exists a $\Theta(1)$ fraction (could be $<\frac12+o(1)$) of the crowd workers who always give responses according to the ground truth function $h^*$, and the learner has access to another verified data source $\expert$. The goal is to learn the underlying Boolean-valued function in such setting with only a small cost per labeled instance.
%{\color{red}We show that} under the {\em semi-verified} learning model of \cite{charika2017learning}, when there exists a $\Theta(1)$ fraction (could be $<\frac12+o(1)$) of the crowd workers who always give responses according to the ground truth function $h^*$, and the learner has access to another verified data source, then it is possible to learn the underlying Boolean function with only a small cost per labeled instance.




%\Jie{Check out the ICML paper; $h(\cdot) = \sign{f(\cdot)}$ is an incorrect argument}

%More formally, we assume there exists an associated class of functions $f\in\F: \X\rightarrow\R$ such that the label of an instance is determined by $h(\cdot) = \sign{f(\cdot)}$. Then, the comparison tag can be thought of as the measurement of the relative distance of two instances $x,x'$ to the decision boundary: $Z(x, x') = \sign{f(x) - f(x')}$. 
%Let $\Z=\{-1,+1\}$ be the set of possible comparison tags, and $\D_\Z$ be the target joint distribution over $\X\times\X\times\Z$, then the zero-error rate function $Z^*(x,x')= \sign{f^*(x) - f^*(x')}$ is such that $\err_{\D_\Z}(Z^*)=0$
%Let $\Z=\{-1,+1\}$ be the set of possible comparison tags such that functions $Z:\X\times\X\rightarrow\Z$. Let $\D_\Z$ be a joint distribution over $\X\times\X\times\Z$, we assume that there exists an underlying zero-error comparison function $Z^*(x,x')= \sign{f^*(x) - f^*(x')}$ such that $\err_{\D_\Z}(Z^*)=0$.
%We further assume that for each pair of instance $(x,x')\in\X\times\X$, there is an underlying zero-error comparison function $Z^*(x,x')$, which outputs $1$ if $x$ is more likely a positive instance than $x'$ is, and $-1$ otherwise.

%In this paper, we focus on the problem of learning Boolean functions when the fraction of correct annotations from the crowd not necessarily be $>\frac{1}{2}+\Theta(1)$. Specifically, we assume the learner has access to two crowd oracles, a label revealing oracle $\oraclelabel$ and a pairwise comparison oracle $\oraclecomp$. The label revealing oracle takes as input an instance and returns its noisy label by querying a random crowd worker from the pool. Similarly, the pairwise comparison oracle $\oraclecomp$ takes as input a pair of instances and answers which one is more likely to be in a specific binary class (e.g. which patient is healthier) by querying a random crowd worker.

%We study the problem of learning Boolean functions, with access to both labels and comparison tags from the crowd. 
%Let $\X$ be the instance space, and $\Y=\{-1,+1\}$ be the set of possible labels. Let $\D$ be the joint distribution over $\X\times\Y$, and denote by $\D_\X$ the marginal distribution on $\X$. A {hypothesis} $h\in\H: \X\rightarrow\Y$ is a Boolean function that maps an instance $x\in\X$ to its label $y$. The error rate of a hypothesis $h$ over $\D$ is defined as $\err_{\D}(h) =\Pr_{(x, y)\sim\D}(h(x)\neq y)$. 

%We consider the {\em realizable} setting, where there exists a hypothesis $h^*\in \H$ such that $\err_{\D}(h^*)=0$, i.e. $y = h^*(x)$. 
%In order to incorporate the pairwise comparisons, we consider a natural extension that has been widely used~\citep{xu2017noise,hopkins2020noise}: for each pair of instance $(x,x')\in\X\times\X$, there is an underlying zero-error comparison function $Z^*(x,x')$, which outputs $1$ if $x$ is more likely a positive instance than $x'$ is, and $-1$ otherwise.
%More formally, we assume there exists an associated class of functions $f\in\F: \X\rightarrow\R$ such that the label of an instance is determined by $h(\cdot) = \sign{f(\cdot)}$. Then, the comparison tag can be thought of as the measurement of the relative distance of two instances $x,x'$ to the decision boundary: $Z(x, x') = \sign{f(x) - f(x')}$.

%\vspace{0.1in}\noindent
%{\bfseries Crowdsourced PAC learning.} \ 
%The key difference between crowdsourced PAC learning and non-crowdsourced one is how the learner gathers the label. Under the non-crowdsourced PAC model, the sample generation oracle first randomly draws $(x, y) \sim \D$, and returns the labeled instance under the passive learning setting or returns only the instance $x$ under the active learning setting. In the latter case, the learner may additionally call a label revealing oracle to obtain the label but no matter how many times the learner makes the call, the label is persistent~\cite{cohn1994improving}. Under the crowdsourced PAC model, the learner only has access to an oracle who can draw instances from $\D_X$. In order to obtain the labels, the learner may assign each instance $x$ to $k$ workers to gather a collection of annotations $h_1(x), \dots h_k(x)$, and may use e.g. majority voting as the final label of $x$. Therefore, in addition to PAC guarantee, another very important evaluation metric of a crowdsourced PAC learning algorithm is the query complexity, namely, the label and comparison queries made to the crowd workers as well as to the trusted expert.

%In this paper, we are interested in the hypothesis classes that are PAC-learnable in realizable setting. Denote by $m_{\epsilon,\delta}$ the sample complexity of learning $\H$ in standard PAC setting. That is, $\forall \epsilon,\delta\in(0,1)$, $m_{\epsilon,\delta}$ is the total number of labeled sample from $\D$ needed to output a hypothesis with error rate $\err_{\D}(h)\leq\epsilon$ with probability $1-\delta$. 
%In this paper, we are interested in crowdsourced learning hypothesis classes that are $(\epsilon,\delta)$-PAC learnable. That is, for any $\epsilon,\delta\in(0,1)$, there exists a learning algorithm that takes as input $m_{\epsilon,\delta}$ correctly labeled instances drawn from $\D$ and returns a hypothesis $h\in\H$ such that, with probability at least $1-\delta$, $\err_{\D}(h)$ is at most $\epsilon$. 
%From the classic VC theory~\citep{anthony2002neural}, we know if there is no additional assumptions on $\H$,
%We will always be interested in crowdsourced learning the {$(\epsilon, \delta)$-PAC learnable classes $\H$} in the paper.
%That is, for any $\epsilon,\delta\in(0,1)$, there exists a learning algorithm which takes as input $m_{\epsilon,\delta}$ correctly labeled instances drawn from $\D$ and returns a hypothesis $h$ such that, with probability at least $1-\delta$, $\err_{\D}(h)\leq\epsilon$. In view of the classic VC theory \cite{anthony2002neural}, it suffices to pick 
%$m_{\epsilon, \delta} = O\(\frac{1}{\epsilon}\(d\log\frac{1}{\epsilon}+\log\frac{1}{\delta}\)\)$,
%\begin{equation}
%m_{\epsilon, \delta} = O\(\frac{1}{\epsilon}\(d\log\frac{1}{\epsilon}+\log\frac{1}{\delta}\)\),
%\end{equation}
%where $d$ is the VC dimension of the hypothesis class $\H$. 
%In our analysis, we will focus on the dependence on $\epsilon$ and take $\delta$ as a constant. Thus, in place of $m_{\epsilon,\delta}$, we will often use a shorthand $m_{\epsilon} = O\(\frac{d}{\epsilon}\cdot\log\frac{1}{\epsilon}\)$.
%\begin{equation}
%m_{\epsilon} = O\(\frac{d}{\epsilon}\cdot\log\frac{1}{\epsilon}\).
%\end{equation}
%We further assume there exist efficient algorithms for the realizable setting. That is, there exists an oracle $\O_\H$ that returns a function $h\in\H$ that is consistent with any input labeled set.

%The learner has access to two noisy crowd oracles, namely, $\oraclelabel,\oraclecomp$. Let $\PL$ be a uniform distribution over all workers in $\oraclelabel$, and $\PC$ be a uniform distribution over all workers in $\oraclecomp$. Thus, $\oraclelabel$ takes as input an instance $x\in\X$ and returns a label $\hat{y}$ by querying a worker $i$ randomly drawn from $\PL$, and $\oraclecomp$ takes as input a pair of instances $(x,x')\in\X\times\X$, and returns a tag $\hat{z}\in\{-1,1\}$ by querying a worker $j\sim\PC$. Note that the crowdsourced setting allows both oracles to return different answers even for identical inputs by querying different crowd workers, which distinguishes it from the standard PAC learning model.
%We are concerned with learning problems in a crowdsourced setting, where the annotations collected from the crowd oracles $\oraclelabel,\oraclecomp$ can be highly noisy. Let $\PL$ be an uniform distribution over all workers in $\oraclelabel$, and $\PC$ be an uniform distribution over all workers in $\oraclecomp$. The oracle $\oraclelabel$ takes as input an instance $x \in \X$ and returns a label $\hat{y}$ by querying a random crowd worker $i$ drawn from distribution $\PL$, while the other oracle $\oraclecomp$ takes as input a pair of instances $(x, x') \in \X \times \X$, and returns a tag $z \in \{-1, 1\}$ by querying a worker $j \sim \PC$.  We remark that by querying the oracle (either $\oraclelabel$ or $\oraclecomp$) multiple times, we may obtain different answers since they are provided by different crowd workers; this is a different feature from standard PAC learning model where the answers are persistent. 



%When the majority of crowd are correct, the problem can be solved by aggregating the crowdsourced data based on majority voting principle. However, when the majority of crowd are incorrect, we can no longer assume that by taking the majority vote over a few random workers we obtain correct annotations according to $h^*$ or $Z^*$.
%In crowdsourced learning setting, the learner has access to two noisy oracles, a label revealing oracle $\oraclelabel$ and a pairwise comparison oracle $\oraclecomp$. 

%\vspace{0.1in}\noindent
%{\bfseries Semi-verified learning model.} \ 
%We study the challenging semi-verified learning model proposed by~\citet{charika2017learning}. That is, there is only a small fraction of the crowd workers that are reliable, i.e. their responses correctly reflect the underlying function $h^*$. More formally, let $\alpha = \Pr_{t\sim\PL}[h_t(x)=h^*(x),\forall x\in\X]$ be the fraction of reliable workers in $\oraclelabel$, and $\beta = \Pr_{t\sim\PC}[Z_t(x,x') = Z^*(x,x'),\forall (x,x')\in\X\times\X]$ be the fraction of reliable workers in $\oraclecomp$. Note that in the semi-verified learning setting $\alpha,\beta$ are potentially $\leq\frac{1}{2}$. Apart from the two crowd oracles, the learner is able to query a trusted oracle $\expert$, who is always able to return the correct label of any given instance or the correct comparison tag of any given pair of instances.
%We assume that there is an $\alpha$-fraction of the crowd workers who are ``reliable'' for providing the labels, i.e. whose responses correctly reflect the underlying function $h^*$, while the remaining $(1-\alpha)$ perform arbitrarily. That is, $\alpha = \Pr_{t\sim\PL}[h_t(x)=h^*(x),\forall x\in\X]$, where $h_t$ denotes the labeling function of the worker $t$ drawn from $\oraclelabel$. Likewise, we assume there is a $\beta$-fraction of the workers in $\oraclecomp$ that are reliable, i.e. $\beta = \Pr_{t\sim\PC}[Z_t(x,x') = Z^*(x,x'),\forall (x,x')\in\X\times\X]$, where $Z_t$ denotes the comparison function of the worker $t$ drawn from $\oraclecomp$. Observe that in our setting, it is possible that $\alpha, \beta < \frac12$.
%In order to handle the large amount of noise in the crowd, we follow the {semi-verified} learning model of \cite{charika2017learning}, and assume that the learner has access to a trusted oracle $\expert$, who is always able to return the correct label of any given instance or the correct comparison tag of any given pair of instances.



%\vspace{0.1in}\noindent
%{\bfseries Overhead of crowdsourcing algorithms.} \ 
%We measure the performance of a crowdsource algorithm by its overall annotation cost with respect to the number of instances need to PAC learn a hypothesis, i.e. $m_{\epsilon, \delta}$.
%which is $m_{\epsilon, \delta} = O\(\frac{1}{\epsilon}\(d\log\frac{1}{\epsilon}+\log\frac{1}{\delta}\)\)$ in view of the classic VC theory \citep{anthony2002neural}.
%In our analysis, we work with constant success probability and concentrate on the dependence on $\epsilon$. Hence, we will often use a shorthand $m_{\epsilon}$ in place of $m_{\epsilon, \delta}$: $m_{\epsilon} = O\(\frac{d}{\epsilon}\cdot\log\frac{1}{\epsilon}\)$.
%Let $\mathcal{A}$ be a learner that takes as input $\epsilon\in(0,1)$ and queries $m_L$ labels from $\oraclelabel$ and $m_C$ comparisons from $\oraclecomp$, as well as a small amount of verified data from $\expert$, such that the learned classifier $h\in\H$ has $\err_\D(h)\leq\epsilon$ with constant probability. We call $m_L$ the {\em label complexity}, and $m_C$ the {\em comparison complexity}. The total number of queries from the crowd will be the sum of them. We define the {\em overhead} of $\mathcal{A}$ to be the ratio of the corresponding queries made by $\mathcal{A}$ to the number of labeled examples needed in the traditional realizable PAC model, i.e. $m_\epsilon$. Then, the {\em labeling overhead} of $\mathcal{A}$ and the {\em comparison overhead} are respectively given by
%\begin{equation}
%\labeloverhead = \frac{m_L}{m_{\epsilon}},\quad \compareoverhead = \frac{m_C}{m_{\epsilon}}.
%\end{equation}
%Note that the number of calls to the trusted oracle $\expert$ is counted separately.

%\begin{equation}
%
%\end{equation}

%Our theoretical analysis is provided based on two theoretical models, as stated below.
%\Jie{I do not think we need to set out the assumptions.}
%Our theoretical analysis will depend on two assumptions, as stated below.
%\begin{assumption}[PAC Learning Model]\label{as:pac}
%	There exists a polynomial-time algorithm $\O_\H$ that $(\epsilon, \delta)$-PAC learns $\H$ using $m_{\epsilon, \delta}$ correctly labeled samples. In addition, there exists a hypothesis $h^*: \X \rightarrow \Y$ with zero classification error over $\D$, and a comparison function $Z^*: \X \times \X \rightarrow \{-1, 1\}$ with zero comparison error over $\D_\Z$.
%\end{assumption}
%\begin{assumption}[Semi-Verified Model]\label{as:noise}
%	There exists an $\alpha$-fraction of the workers in distribution $\PL$, and a $\beta$-fraction of the workers in distribution $\PC$.	Here $0<\alpha,\beta<\frac{1}{2}+o(1)$ are given to the learner. In addition, the learner has access to a trusted oracle $\expert$ that guarantees to provide correctly labeled instance drawn from $\D$ for any $x\in\X$, and correctly tagged pair drawn from $\D_\Z$ for any $(x,x')\in\X\times\X$.
%%	The fraction of the reliable workers in distribution $\PL$ is $\alpha$, and the fraction of the reliable workers in distribution $\PC$ is $\beta$. 
%%	That is, for any given instance, each time $\oraclelabel$ returns its correct label with probability at least $\alpha$; and for any given pair of instances, each time $\oraclecomp$ returns their correct comparison tag with probability at least $\beta$. 
%\end{assumption}



%Specifically, consider there exist a large pool of crowd workers in $\oraclelabel$, at least a noticeable fraction, i.e. $\alpha$, of which are {\em perfect}, that is, they always label according to the target function $h^*$. Likewise, in $\oraclecomp$, at least a $\beta$ fraction of the workers would always tag according to the target function $Z^*$.
%Although we allow the crowd oracles to be highly noisy, we assume there exist a noticeable fraction of the crowd workers in the pool are {\em perfect}, i.e. they always label according to the target function $h^*$. 
%Then, the underlying Boolean function is learnable with a $O(\frac{1}{\alpha}+\frac{1}{\beta})$ overhead.
%\Shiwei{perfect labelers?}

%\Shiwei{Assumption: since all the sample instances are drawn i.i.d. from the distributions, a pair $(x_i,x_j)$ that is a good test case for workers in $\PC$ does not necessarily mean that $(x_i,x_\ell), \forall \ell\neq j$ is also a good test case. Actually, we will assume the difficulties between pairs of instances to be independent. Assume that the difficulty is proportional to the distance between two instances $x_i,x_j$, if $x_i$ is very close to $x_j$ such that the order of them is hard to tell, making it a more difficult pair to compare, it does not necessarily mean that $x_i$ will also be close to any other instance $x_\ell$, as their positions are independent.}

